Positional Encoding as Spatial Inductive Bias in GANs

SinGAN shows impressive capability in learning internal patch distribution despite its limited effective receptive field. We are interested in knowing how such a translation-invariant convolutional generator could capture the global structure with just a spatially i.i.d. input. In this work, taking SinGAN and StyleGAN2 as examples, we show that such capability, to a large extent, is brought by the implicit positional encoding when using zero padding in the generators. Such positional encoding is indispensable for generating images with high fidelity. The same phenomenon is observed in other generative architectures such as DCGAN and PGGAN. We further show that zero padding leads to an unbalanced spatial bias with a vague relation between locations. To offer a better spatial inductive bias, we investigate alternative positional encodings and analyze their effects. Based on a more flexible positional encoding explicitly, we propose a new multi-scale training strategy and demonstrate its effectiveness in the state-of-the-art unconditional generator StyleGAN2. Besides, the explicit spatial inductive bias substantially improve SinGAN for more versatile image manipulation.

==> arxiv_sections/__latexindent_temp.tex <==
% !TEX root = ../main.tex

SinGAN shows impressive capability in learning internal patch distribution despite its limited effective receptive field.
%
We are interested in knowing how such a translation-invariant convolutional generator could capture the global structure with just a spatially \iid~input.
%
In this work, taking SinGAN and StyleGAN2 as examples, we show that such capability, to a large extent, is brought by the implicit positional encoding when using zero padding in the generators.
%
Such positional encoding is indispensable for generating images with high fidelity. The same phenomenon is observed in other generative architectures such as DCGAN and PGGAN. 
%
We further show that zero padding leads to an unbalanced spatial bias with a vague relation between locations.
% 
To offer a better spatial inductive bias, we investigate alternative positional encodings and analyze their effects.
%
Based on a more flexible positional encoding explicitly, we propose a new multi-scale training strategy and demonstrate its effectiveness in the state-of-the-art unconditional generator StyleGAN2. 
%
Besides, the explicit spatial inductive bias substantially improve SinGAN for more versatile image manipulation.


\if 0
% Spatial structure, including spatial anchors and transformation between adjacent locations, is one of the most essential pursuits when it comes to image generation.
% Recent works find that convolutional networks in high-level tasks (\eg, image classification and detection) are not translation-invariant in some experiments. 
%
% However, how convolutional generators capture spatial information lacks a comprehensive study.
Recent popular SinGAN learns the internal patch distribution through its limited effective receptive field.
% Existing GAN literature reveals little about how spatial structure is captured and its effects on current generative models.
%
However, we are curious about how the translation-invariant convolutional generator can capture the global structure with a spatial \iid~input.
%
In this work, taking SinGAN and StyleGAN2 as examples, we demonstrate the commonly used asymmetric zero padding injects spatial information in generators theoretically and experimentally.
%
Furthermore, this phenomenon is also spotted in various generator architectures, like DCGAN and PGGAN. 
%
% When it comes to the diversity and manipulation in StyleGAN2, we discover the asymmetric padding limits the generator to fewer structures in the training distribution and makes the border of outputs uncontrolled by the input signal.
%
% Besides the asymmetric zero-padding, learnable fixed noise in StyleGAN2, traditional Cartesian spatial grid and sinusoidal positional embedding can also introduce spatial information with implicit or explicit properties of spatial anchors and transformation between locations.
%
% With different strategies to offer positional embedding, we explore a solution to remove all of the paddings in StyleGAN2 and demonstrate its generalization in other unconditional GANs.  
%
% In the end, our more effective MSStyleGAN and SPE-SinGAN indicate that a missing keypoint in generative models is to adopt an appropriate positional embedding with task-oriented spatial information.
%
% \bad{This general observation} indicates spatial information is essential for the translation-invariant generators to guarantee a faithful structure. 
% This general observation indicates 
%
However, the implicit positional encoding introduced by the asymmetric zero-padding leads to an unbalanced spatial inductive bias with a vague relation between some locations.
% 
To offer a better strategy for encoding positional information, we investigate different explicit positional encodings and comprehensively analyze their effects.
%
Based on the flexible explicit positional encoding, we propose a new multi-scale training strategy (MUSTPE) and demonstrate its effectiveness in the current state-of-the-art unconditional generator StyleGAN2. 
%
% The significant improvement in SinGAN and MSStyleGAN with suitable positional encodings indicates introducing appropriate spatial inductive bias to convolutional generators is an important element missing from current literature.
Besides, thanks to the explicit spatial inductive bias, SinGAN can easily handle more challenging cases with different requirements. 
% By making full use of the structure and texture information across different scales, our MSStyleGAN can deal with multi-scale synthesis with lower FID at each scale.
%
% Furthermore, comprehensive experiments demonstrate that how to introduce appropriate spatial information to convolutional generators is a missing keypoint in current literature.
% In this study, we show that commonly used asymmetric zero-padding serves as a kind of important implicit positional embedding leaking spatial information to convolutional generative networks but induces networks to overfit to several structures of training distribution and make the border of outputs unconstrained in our \bad{padding-free test} for StyleGAN2. 
%
% Besides asymmetric zero-padding, learnable fixed noise, traditional Cartesian spatial grid map, and sinusoidal positional embedding can also introduce spatial structures with different valuable properties, like consistent transformation between neighboring locations and natural generalization to changing scales.
%
% We investigate the phenomenon of leaking spatial information by asymmetric zero-padding and different positional embedding strategies from traditional DCGAN and PGGAN to current  popular StyleGAN2 and SinGAN, which also reveals how SinGAN captures global structure with limited effective receptive field.
%
% Furthermore, a general solution with sinusoidal positional embedding is proposed for general convolutional GANs to remove asymmetric padding. 
%
% In the end, our more effective MSStyleGAN and SPE-SinGAN indicate that a missing keypoint in generative models is to adopt an appropriate spatial structure with task-oriented geometry priors.

\fi

